Towards Model-Size Agnostic, Compute-Free, Memorization-based Inference of Deep Learning

The rapid advancement of deep neural networks has significantly improved various tasks, such as image and speech recognition. However, as the complexity of these models increases, so does the computational cost and the number of parameters, making it difficult to deploy them on resource-constrained devices. This paper proposes a novel memorization-based inference (MBI) that is compute free and only requires lookups. Specifically, our work capitalizes on the inference mechanism of the recurrent attention model (RAM), where only a small window of input domain (glimpse) is processed in a one time step, and the outputs from multiple glimpses are combined through a hidden vector to determine the overall classification output of the problem. By leveraging the low-dimensionality of glimpse, our inference procedure stores key value pairs comprising of glimpse location, patch vector, etc. in a table. The computations are obviated during inference by utilizing the table to read out key-value pairs and performing compute-free inference by memorization. By exploiting Bayesian optimization and clustering, the necessary lookups are reduced, and accuracy is improved. We also present in-memory computing circuits to quickly look up the matching key vector to an input query. Compared to competitive compute-in-memory (CIM) approaches, MBI improves energy efficiency by almost 2.7 times than multilayer perceptions (MLP)-CIM and by almost 83 times than ResNet20-CIM for MNIST character recognition.

==> sections/background.tex <==
\section{Related Work}
In recent years, there has been a growing interest in reducing the computational overhead of neural networks. This has been achieved through various methods, such as reducing the model size or applying attention mechanisms to smaller portions of the input. One noteworthy work, published in 2014, aimed to combine Recurrent Neural Networks (RNNs) with an attention mechanism \cite{mnih2014recurrent}. Specifically, this network was trained to understand where to focus at each time-step, and ultimately to classify the inputs at the last time-step.

In this section, we will start by explaining the fundamentals of RNNs, we will then go through the attention mechanism, and we will also explore different approaches to reduce the model size. However, manually tuning the many hyperparameters required by these networks can be a challenge. To address this issue, we will introduce the Bayesian Optimization algorithm. Finally, we will go through a general overview of popular datasets used in classification.

\subsection{Overview of RNN}
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{resources/lstm.png}
        \caption{LSTM unit}
        \label{fig:lstm}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{resources/transformers.png}
        \caption{Transformer unit}
        \label{fig:transformers}
    \end{subfigure}
    \caption{}
    \label{fig:rnn-units}
\end{figure}

Recurrent Neural Networks (RNNs) are a fundamental tool for sequence modeling, especially in Natural Language Processing (NLP), where each sentence is composed of a series of words that are naturally correlated with each other. However, RNNs suffer from the vanishing gradient problem, which occurs when gradients in the network become too small as they propagate backward through the layers \cite{hochreiter2001gradient}. This problem is particularly severe when dealing with long input sequences, since each layer of the RNN has a time-step loop calculation and the number of time-steps is equal to the length of the input sequence \cite{fang2021survey}. To address this issue, Long Short Term Memory networks (LSTMs) were introduced by Hochreiter \& Schmidhuber in 1997 \cite{hochreiter1997long}.

LSTMs are a type of gated algorithm, where each gate controls the flow of information through the network \cite{fang2021survey}. The standard LSTM network has three gates: an input gate, a forget gate, and an output gate \cite{adaloglou2020rnn} [Fig.~\ref{fig:lstm}]. The input gate determines the input of the current time-step and updates the internal state with respect to the previous time-step. The forget gate determines whether to retain or forget information. Lastly, the output gate is based on the internal state but filtered through the other gates of the LSTM.

LSTMs have already achieved remarkable results in various fields, including speech recognition, language modeling, translation, and image captioning \cite{olah2015understanding}. The ability of LSTMs to solve the long-term dependencies problem has been critical in achieving these results. Combining attention mechanisms with LSTMs has been another major breakthrough in the state-of-the-art. The next section will be dedicated to the attention mechanism.

\subsection{Attention mechanism}
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{resources/attention-alignment.png}
        \caption{Example of an attention heat-map}
        \label{fig:attention-heatmap}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{resources/obama-embedding.png}
        \caption{Example of euclidean distance between embeddings}
        \label{fig:eucledian-distance-embeddings}
    \end{subfigure}%
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{resources/obama-embeddings-2.png}
        \caption{Example of similarity between sentences}
        \label{fig:sentences-similarity-embeddings}
    \end{subfigure}
    \caption{}
    \label{fig:rnn-units}
\end{figure*}

The attention mechanism refers to a network's ability to assign varying degrees of importance to different parts of the input. Attention can be either implicit or explicit \cite{adaloglou2020normalization}. Deep neural networks, being complex function approximators, implicitly learn to ignore irrelevant input during the training process. However, explicit attention involves actively requesting the network to weigh the significance of the input based on multiple factors. In this case, learning parameters are added to the network with the sole purpose of determining the importance assigned to specific subsets of the input.


Attention can be computed globally or locally on the input sequence \cite{adaloglou2020normalization}. Global attention involves considering the entire input sequence, while local attention involves examining only a subset of the input sequence. Local attention is less computationally expensive but requires making "hard" decisions about which parts of the input to focus on at each time step.

Attention can be visually represented with a heat map. In Fig.~\ref{fig:attention-heatmap}, we show an example of a translation attention mechanism between English and French. The heat map illustrates the attention that each word receives with respect to its corresponding translation in the other language. In the highlighted area, the model learned to swap the order of words in translation.

We can also define self-attention, which is attention over the same sequence of words \cite{adaloglou2020normalization}. Self-attention focuses on the score between the same sequence of elements instead of an input-output sequence. Self-attention is the foundation of the state-of-the-art NLP algorithm: Transformers \cite{vaswani2017attention}.

\subsection{Basic concepts of Transformers}
Transformers are currently considered the state-of-the-art in Natural Language Processing (NLP) and have been widely used since 2020 for a variety of tasks ranging from NLP to computer vision \cite{adaloglou2021transformer}. They rely heavily on the self-attention mechanism and utilize tokenization and word embeddings.

\subsubsection{Tokenization}
Tokenization is the process of breaking down a sentence into individual words, without taking their positions into account. This means that the input sentence becomes a set of words (tokens) without any positional significance within the set. However, in the case of Transformers, positional encodings are necessary after tokenization, as the order of words naturally carries importance in a sentence.

\subsubsection{Word embeddings}
An embedding is generally a representation of a symbol in a distributed, low-dimensional space of continuous-valued vectors. In other words, a word can be represented as a fixed-length vector of real numbers. \texttt{Word2Vec} \cite{mikolov2013distributed} is a network that learns a vector representation for each word and has been widely used for various NLP tasks requiring word embeddings, as it has been demonstrated that it generates superior word embeddings for most general NLP tasks compared to other approaches \cite{wang2018comparison}. This network can not only learn an embedding for each word, but has also shown that the mathematical relationships between embeddings is correlated with semantic relationships \cite{kusner2015word}. For example, when represented in a 3D space, vectors with similar Euclidean distances also tend to be semantically related, as shown in Fig.\ref{fig:eucledian-distance-embeddings}. Fig.~\ref{fig:sentences-similarity-embeddings} also shows that the embeddings can help detect entire similar sentences: $D_1$ and $D_2$ are equally similar to $D_0$.

\subsubsection{Self-Attention and Efficacy}
Transformers combine self-attention, word embeddings, tokenization, and a few other techniques, resulting in the architecture depicted in Fig.~\ref{fig:transformers}. They are effective for several key reasons \cite{adaloglou2021transformer}:
\begin{itemize}
    \item Each block has distributed and independent representations, providing various contextualized representations for the input.
    \item Self-attention is the primary factor responsible for providing meaning that is highly dependent on the context.
    \item Multiple encoder and decoder blocks enable a more abstract representation of the state.
    \item Skip connections facilitate a combination of high- and low-level information. While not unique to Transformers, this is one of the reasons why they work so well.
\end{itemize}

\subsection{Model Size Reduction Techniques}
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/pruning.png}
        \caption{BBP vs BW}
        \label{fig:pruning}
    \end{subfigure}%
    \begin{subfigure}{0.2231\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/linear-quantizer.png}
        \caption{Linear quantizer}
        \label{fig:linear-quantizer}
    \end{subfigure}%
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/log-quantizer.png}
        \caption{Logarithmic quantizer}
        \label{fig:log-quantizer}
    \end{subfigure}%
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/non-linear-quantizer.png}
        \caption{Non-linear quantizer}
        \label{fig:non-linear-quantizer}
    \end{subfigure}
    \caption{}
    \label{fig:rnn-units}
\end{figure*}


Reducing the size of a neural network model is often desirable due to limited computational resources and memory constraints. In literature, various techniques have been proposed for reducing the model size, with the main focus being on reducing the number of parameters of the network. However, some of these techniques can also be applied to reduce the size of the inputs and outputs of our model.

\subsubsection{Network pruning}
Network pruning is a technique that takes advantage of the overparameterization of neural networks. In fact, networks have usually a large amount of weights, and most of them result in redundancy. Hence, they can be removed (i.e. set to zero) maintaining the original accuracy or worsening it in a negligible way \cite{sze2017efficient}.

One popular technique for model size reduction is network pruning. This technique takes advantage of the overparameterization of neural networks, where many of the weights in a network result in redundancy. Hence, pruning techniques can be used to remove some of these redundant weights, resulting in a smaller network with minimal impact on its accuracy \cite{sze2017efficient}. Additionally, pruning techniques can also be used to harness the sparsity of weight matrices, where weights that are equal to zero or close to zero can be pruned and eliminated, reducing the space and complexity of the network \cite{qi2021accommodating}. Two commonly used pruning techniques are block-balanced pruning (BBP) \cite{li2020efficient} and block-wise pruning (BW) \cite{narang2017block}, which can be applied to reduce the size of the weight matrices, as shown in Fig.~\ref{fig:pruning}.

Apart from weight pruning, the same techniques can also be applied to inputs of the neural network. In many cases, the inputs to a neural network may consist of sparse matrices or sparse vectors, where elements close to zero can be eliminated at the source, reducing the size of the input to the model.

\subsubsection{Quantization}
Quantization is the process of mapping data to a smaller set of quantization levels, with the goal of minimizing the error between the reconstructed and original data. The precision of the quantization increases with the number of quantization levels, which can be represented by the number of bits, given by the equation:
\begin{equation}
b = \log_2(q)
\end{equation}

where $q$ is the number of quantization levels and $b$ is the number of bits.

There are various methods to quantize data \cite{sze2017efficient}, such as uniform quantization levels, where each level is separated by an equal distance [Fig.~\ref{fig:linear-quantizer}], logarithmic function to map the data to quantization levels with varying distances [Fig.~\ref{fig:log-quantizer}], or a more intricate mapping function [Fig.~\ref{fig:non-linear-quantizer}], where the quantization levels are determined or learned from the data using approaches like k-means clustering.

Research focuses on reducing the precision and size of several factors, depending on the project goals. For hardware co-design of a neural network, the precision is reduced on weights more than on the activation functions, as the weights directly impact the storage capacity. Some works have also looked at quantization on the activation functions, while others have explored quantization only during inference. The latter approach is useful to avoid vanishing gradient descent, as it is easier to reach zero when the precision of weights is decreased. In our case, we applied quantization on inputs and outputs, training and testing the original network in software.

The quantization scheme during inference is usually deterministic, but sometimes stochastic quantization could allow a neural network to explore more \cite{gholami2021survey}. For example, the Int operator of works like \cite{gupta2015deep,chen2020statistical} uses a stochastic quantization method given by:
\begin{equation}
    \text{Int}(x) = \begin{cases} 
      \lfloor x \rfloor & \text{with probability } \lceil x \rceil - x, \\
      \lceil x \rceil & \text{with probability } x - \lfloor x \rfloor.
   \end{cases}
\end{equation}

Quantization can be either \emph{simulated} or \emph{integer-only}, which refers to the actual coding used when doing arithmetic operations. The former saves the model in a low-precision fashion, quantized with the number of levels decided a priori, but the operations are still carried on through floating-point values. Hence, before applying the operations, the values must be dequantized, usually done with a map. Instead, integer-only quantization performs the arithmetic operations using quantized values, which can be either fixed points or integers \cite{gholami2021survey}.

Finally, quantization can be performed equally throughout the model, or different levels of quantization can be applied to different layers of the model. For example, a neural network with two hidden layers could have linear quantization best suited for the first layer, and non-linear quantization, like logarithmic or more complex, for the second layer. In this case, the quantization applied is called \emph{mixed-precision quantization} \cite{gholami2021survey}.

Non-linear quantization is suitable for many case studies, but it usually needs to learn in advance or on the run how the quantization must be performed. Two examples of non-linear quantization are the KMeans Clustering quantizer or the Lloyd-Max quantizer. KMeans Clustering clusters the weights into different groups and uses the centroid of each group as quantized values during inference, as shown in Eq. \ref{eq:vector-quantization-kmeans}:
\begin{equation}\label{eq:vector-quantization-kmeans}
    \min_{c_1,\ldots,c_k} \sum_{i}||w_{i} - c_{j}||^2
\end{equation}

Here $i$ is the index of weights in a vector, $c_1,\ldots,c_k$ are the $k$ centroids found by the clustering, and $c_j$ is the corresponding centroid to $w_i$. The number of clusters, denoted as $k$, can be predetermined and corresponds to the number of quantization levels \cite{gholami2021survey}. On the other hand, the Lloyd-Max algorithm aims to adjust the quantization values such that the probability density function's area is the same for each quantization step. As a result, this quantizer has dense quantization steps in areas with high probability density and wide quantization steps in areas with low probability density \cite{gong2014compressing}. While KMeans Clustering is more suitable if our goal is to group similar weights, Lloyd-Max is crucial when our objective is to retain the most possible information after quantization. This concept is similar to applying logarithmic quantization to weights that are distributed with a Gaussian distribution, where denser weights result in closer quantization steps [see Fig.~\ref{fig:log-quantizer}].

\subsection{Bayesian Optimization}
Bayesian Optimization is an algorithm commonly used for optimizing functions that take minutes or hours to evaluate and are not suited for manual configuration of hyperparameters. This heuristic is most effective for optimizing continuous domains with less than 20 dimensions and can tolerate stochastic noise in function evaluations \cite{frazier2018tutorial}. Bayesian optimization is focused on solving the general problem:
\begin{equation}
    \max_{x\in A} f(x)
\end{equation}

In other words, if we have a function that takes a set of inputs (e.g., hyperparameters) and produces an output (e.g., accuracy of a network), BO aims to find the optimal set of inputs that maximizes the output of the function. By doing so, it allows us to find the hyperparameters that result in the best possible accuracy for our network.



\subsection{Popular Datasets}
In order to compare our accuracy to the existent ones for different models and different datasets, it is wise to consider the top accuracy for some of the most common datasets available for machine learning. We will mostly focus on image datasets for classification purposes, mentioning their complexity and their best accuracy \cite{sze2017efficient}.

\subsubsection{MNIST}
MNIST is the easiest and least complex dataset, consisting of 28x28 grayscale images of handwritten digits from 0 to 9. The first convolutional neural network ever developed, LeNet-5 \cite{lecun1998gradient}, was able to achieve an accuracy of 99.05\% when MNIST was first introduced. Since then, the accuracy has increased to 99.91\% \cite{an2020ensemble}, according to \cite{mnistaccuracy}, and it is considered nowadays a fairly easy dataset.

\subsubsection{FashionMNIST}
FashionMNIST also consists of 28x28 grayscale images, but instead of handwritten digits, it contains images of clothing items, which are considered more challenging for neural networks \cite{xiao2017fashion}. When FashionMNIST was introduced, it achieved an accuracy of 89.7\% in the original paper. Recently, the \texttt{pFedBreD} model achieved an accuracy of 99.06\% \cite{shi2022personalized}, which is currently the highest achieved accuracy for FashionMNIST, according to \cite{fashionmnistaccuracy}.

\subsubsection{CIFAR}
CIFAR is a slightly more complex dataset, consisting of 32x32 colored images of various subjects (RGB images with 3 channels). \texttt{CIFAR-10} specifically contains 10 mutually exclusive classes, similarly to MNIST and FashionMNIST. The first network used on CIFAR-10 achieved an accuracy of 64.84\%. Since then, the accuracy has increased to 99.61\% \cite{yuan2021florence}, according to \cite{cifar10accuracy}.

\subsubsection{ImageNet}
ImageNet is a much larger dataset containing colored images of size 256x256 and 1000 classes. The highest top-5 error accuracy achieved on ImageNet was 99.02\% \cite{yuan2021florence}, according to \cite{imagenetaccuracy}.

==> sections/conclusions.tex <==
\section{Conclusion}
In this paper, we have discussed Memory-Based Inference (MBI) and presented some notable results regarding its accuracy. One of the significant advantages of this approach is its exceptional scalability towards very deep neural networks, regardless of the model's final size.

We have presented various trained table structures, as well as distance metrics, to be considered when using MBI. Furthermore, we have simulated a hardware implementation by introducing some noise and plotting the possible decline in overall accuracy.

We are confident this will be a first step towards a novel approach, as neural networks are constantly increasing in size and depth.

==> sections/content-addressable-search.tex <==
\section{High-Performance Content Addressable Search}

==> sections/future.tex <==
\section{Future Work}
As MBI is a first attempt at a novel approach, there is considerable room for improvement. Here are some specific areas that we plan to focus on:

\subsection{Dataset Complexity}
Initially, we focused on training and testing the model on the MNIST dataset due to its speed and simplicity. This allowed us to identify the major pros and cons of our approach. We also conducted tests on two additional datasets to measure the accuracy drop from standard inference to MBI. However, further work is needed to improve performance on different datasets. Specifically, we need to fine-tune the hyperparameters for each dataset, as well as explore the suitability of different network architectures. This will help us improve the accuracy and generalizability of our approach across various datasets.

\subsection{Distance Function}
In this paper, we utilized the distance function presented in Eq.~\ref{eq:noised-distance}. This approach involves a simple noised and weighted Manhattan distance that allows for ease of hardware implementation. However, there is still room for further research to fine-tune a more appropriate distance function that can potentially enhance the performance of the model.

\subsection{Interpolation}
Our MBI approach requires finding the closest input row in the table to the input test data. Once found, the saved output will be extracted from the table and considered as a solution. However, due to the high space complexity of all possible output vector combinations, the trained table can only store a limited amount of output vectors. This limitation means that our model can only predict outputs that have already been stored in the table, and it cannot predict \emph{new} outputs.

As a consequence, the accuracy of two equal-sized tables may differ depending on the number of output combinations possible. The more output combinations that are possible, the lower the accuracy will be.

One possible solution would be to look up both the upper-closest and lower-closest row, extract the outputs of both rows, and generate a new output by calculating the weighted mean of the two outputs based on the relative distance between the test input and the inputs in the table. However, further testing is required to determine whether this approach can improve the accuracy of the MBI model.

==> sections/introduction.tex <==
\section{Introduction}
Recurrent Neural Networks (RNNs) have been a remarkable breakthrough in the realm of deep learning, offering algorithms to effectively model input sequences \cite{fang2021survey}. Among the types of RNNs, Long Short-Term Memory networks (LSTMs) have demonstrated exceptional performance in a multitude of domains \cite{olah2015understanding}.

Attention mechanism revolutionized the computational complexity of neural networks \cite{adaloglou2020normalization}, and paved the way for the current state-of-the-art network for Natural Language Processing (NLP) \cite{vaswani2017attention}, propelling the field to new heights.

By combining the attention mechanism with recurrent neural networks, some researchers have provided the network with sufficient time to grasp where to focus on the input. The Recurrent Attention Model (RAM) \cite{mnih2014recurrent} embodies this concept, yielding highly favorable outcomes.

Our work expands on RAM by introducing Memory-Based Inference (MBI). The main goal of this paper is to create an inference model that is independent of its size or depth, making the network's complexity irrelevant. The development of more intricate models results in higher computational costs and a larger number of parameters, making it challenging to deploy inference on devices with limited resources. However, with MBI, only the size of the model's inputs and outputs require attention, as the network can be treated as a black box. This approach also provides excellent scalability from an inference perspective. Assuming that the input and output sizes remain constant, any changes to the network will only affect accuracy, not inference.

This paper is organized into [NUMBER] sections. First, we introduce related works found in the literature. Next, we detail the structure of our model and our methodology. Finally, we conclude with the results and performance analysis.

==> sections/methodology.tex <==
\section{Methodology}\label{sec:methodology}
Our approach aims to create an inference system that is independent of the size or depth of the neural network model. This means that the inference workload remains constant regardless of the number of layers or model parameters, and instead depends only on the input and output size.

We developed our methodology based on the Recurrent Attention Model (RAM) \cite{mnih2014recurrent}. This model uses a combination of Recurrent Neural Network (RNN) and attention mechanism to selectively focus on a smaller window of the input image and classify it. The network is trained to identify where to focus at each time-step to optimize the final classification of the input image.

In the following sections, we will first introduce the original network as proposed by Mnih et al. and we will then go through the steps taken to build Memory-Based Inference (MBI) on top of that.

\subsection{RAM Structure}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{resources/ram.png}
    \caption{RAM model}
    \label{fig:RAM-model}
\end{figure*}

This is a recurrent neural network with an attention mechanism designed to classify input images. The attention mechanism employs a ``glimpse networ'' that extracts a smaller window of the input image for further processing, while recurrence is achieved through a ``core network'' that processes the hidden state vector from the previous time-step and outputs a new hidden state vector related to the current time-step. At each time-step, a ``location network'' computes a new location vector that is used in the next time-step to focus on a specific location. We will now provide a detailed explanation of each step, and we will refer to Fig.~\ref{fig:RAM-model} for the nomenclature and visualization of the model.

\subsubsection{Glimpse network}\label{sec:glimpse-network}
In the original paper \cite{mnih2014recurrent}, each time-step of the network is referred to as a ``glimpse''. To avoid misunderstandings, we will keep using this terminology. The glimpse network takes an input image and a location vector and extracts subsets of the image based on the coordinates specified in the location vector. The extraction process is important to understand the fine-tuning we applied to the hyperparameters:
\begin{enumerate}
    \item Assume we have a 28x28 pixel input image and we want to extract 3x3 pixel subset of the image. The location vector will tell the network where to focus on, and then the network will extract a 3x3 pixel \emph{patch} from it. In Fig.~\ref{fig:RAM-model}, the extracted patch is represented by the innermost blue rectangle of the glimpse sensor.
    \item The network then extracts a larger patch than the previous one, based on the \emph{glimpse scale} hyperparameter that we define. For instance, if the glimpse scale is 2, the network extracts a patch large twice the previous one, i.e. a 6x6 pixel patch. After extracting it, the patch is then downsized again to 3x3 pixels, using for example average pooling. As a result, the second patch covers a larger input area but with lower resolution (it remains 3x3 pixels in size).
    \item This process is repeated a fixed number of times, specified by the \emph{patches number} hyperparameter. Once all patches have been extracted, they are flattened and stacked to form the \emph{patch vector}. The patch vector therefore consists of flattened patches of the same size but with decreasing resolution.
\end{enumerate}

The \emph{patch size} hyperparameter determines the size of the patches in pixels. Therefore, the whole size of the patch vector is given by Eq.~\ref{eq:patch-vector-size}, which is crucial for compressing the input size of the look-up table for memory-based inference:
\begin{equation}\label{eq:patch-vector-size}
    S = patch\_size \times patches\_number
\end{equation}

For grayscale images like MNIST, there is only one channel. For images with multiple channels, such as RGB images in CIFAR-10, the operation is applied channel-wise, and the channels are stacked as individual patches. In this case, the new size of the patch vector would be given by Eq.~\ref{eq:patch-vector-size-channels}:
\begin{equation}\label{eq:patch-vector-size-channels}
    S = patch\_size \times patches\_number \times channels
\end{equation}

After passing through some hidden layers, the glimpse network generates the glimpse vector $g$. From a broader perspective, the glimpse network functions as a mechanism of attention that focuses on part of the input image provided to the network.

\subsubsection{Core network}
The core network is responsible for computing the hidden state of each glimpse in the model. This hidden state is represented by the vector $h_t$ shown at Fig.~\ref{fig:RAM-model}. The core network combines the hidden state vector of the previous glimpse $h_{t-1}$ with the output of the glimpse network $g_t$, and produces the new hidden state $h_t$. The ultimate goal of the core network is to generate the hidden state for each glimpse, which contains both the current attention information and the information from the previous hidden states.

\subsubsection{Location network}
The location network generates a new location vector based on a probability function using the current hidden state. In other words, it determines where the model should focus its attention in the next glimpse.

\subsubsection{Classification network}
The classification network computes classifications at each glimpse, but for the purposes of classification, they are only considered in the final glimpse.

\subsubsection{Inputs and outputs}\label{sec:glimpse-inputs-outputs}
As you could have already deduced, each glimpse could be considered as a black-box with three input vectors and three output vectors. Memory-based inference will make use of a trained look-up table composed only by these inputs and outputs. Therefore, the size of the look-up table will depend on the size of the inputs and outputs. Specifically, we have:
\begin{itemize}
    \item Inputs:
    \begin{itemize}
        \item Current location vector $l_t$: this is a 2-element vector that indicates the $x$ and $y$ coordinates. It changes with each glimpse.
        \item Input image: this is the sample from the dataset and remains constant for each glimpse. We anticipate here that we mostly used the MNIST dataset, which consists of 28x28 grayscale images with one channel.
        \item Previous hidden state vector $h_{t-1}$: this is a $N$-element vector. In the original paper, it was a 256-element vector with 32-bit floating-point numbers. For the first glimpse, it is initialized to all zeros.
    \end{itemize}
    \item Outputs:
    \begin{itemize}
        \item Current hidden state vector $h_t$: this has the same structure as the correspondent input.
        \item Next location vector $l_{t+1}$: this has the same structure as the correspondent input. If it is computed in the last glimpse, it is ignored.
        \item Prediction $a_t$: this is a 1-element vector (scalar) representing the class chosen by the network.
    \end{itemize}
\end{itemize}

\subsection{Hyperparameters Tuning}
\begin{table*}[t]
    \begin{center}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
            \toprule
            \textbf{\# glimpses} & \textbf{patch size} & \textbf{glimpse scale} & \textbf{\# patches} & \textbf{\emph{h} quant.} & \textbf{\emph{p} quant.} & \textbf{\emph{h} size} & \textbf{added layers} & \textbf{inference acc.} \\
            \midrule
            5 & 4x4 & 4 & 3 & 1 & 2 & 64 & 1 & 96.00\% \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Hyper-parameters for baseline.}
    \label{tab:hyperparameter-baseline}
\end{table*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/graphs/patch.png}
        \caption{}
        \label{fig:patch}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/graphs/model_size.png}
        \caption{}
        \label{fig:size}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=.95\linewidth]{resources/graphs/quantization.png}
        \caption{}
        \label{fig:quantization}
    \end{subfigure}
    \caption{Accuracy differences isolating one hyper-parameter at a time.}
    \label{fig:graphs}
\end{figure*}

We had to adjust multiple hyperparameters while balancing accuracy with table size. Ultimately, we settled on a \emph{baseline configuration}, which is presented in Tab.~\ref{tab:hyperparameter-baseline}. We then implemented memory-based inference on top of this configuration.

In this paper, we focus on examining the impact of individual hyperparameters on accuracy. To do so, we isolated one hyperparameter at a time and analyzed the differences in accuracy resulting from changing the value of that parameter [Fig.~\ref{fig:graphs}]. In the following sections, we will delve into each hyperparameter and discuss its role in more detail.

\subsubsection{Number of glimpses}
The number of glimpses refers to the total number of time-steps taken for each sample (input image). In contrast to other types of recurrent neural networks (RNNs), the number of time-steps in this case is not dependent on the length of the input sequence, since there is no input sequence involved. Instead, each input image is treated independently as a separate sample, and processed accordingly. The purpose of the recurrence in this context is to provide the network with enough time to determine where to focus its attention. The initial focus is selected at random (using a uniform random distribution to choose the starting coordinate), after which it is refined based mostly on the patches with lower resolution, which can indeed capture a larger portion of the image. 

Each glimpse is represented by a row of inputs and outputs from the look-up table. Therefore, fewer glimpses will result in a smaller table. In Figure~\ref{fig:patch}, the red line indicates the accuracy achieved by different numbers of glimpses.

\subsubsection{Hyperparameters for the patch vector}
In Sec.~\ref{sec:glimpse-network}, we discussed the extraction of the patch vector $p$ within the glimpse network. The length of this vector is determined by several hyperparameters: patch size, glimpse scale, number of patches, and, in some cases, the number of input image channels. The total length of the patch vector can be calculated using the formula provided in Eq.~\ref{eq:patch-vector-size-channels}.

It may seem puzzling why the size of the patch vector matters since it is not included in the glimpse inputs, as we have previously noted in Section~\ref{sec:glimpse-inputs-outputs}. However, it is important to understand that we saved the patch vector $p$ in our table rather than the input image because it represents a focused variation of the input image. We will elaborate more on the table later in the paper.

To visualize the impact of these hyperparameters on accuracy, we generated Fig.~\ref{fig:patch}, which shows the accuracy of our model for various patch sizes (blue), glimpse scales (green), and patch numbers (purple). It is worth noting that we do not have data for patch numbers greater than 5 because the resulting model was taking too long to train.

\subsubsection{Model Structure}
We have made some modifications to the model structure, balancing model size and accuracy. The following factors were considered:
\begin{itemize}
    \item Hidden state vector length: The length of the hidden state vector $h$ is directly related to the size of the final table. However, reducing the vector size diminishes the state information and thus affects the accuracy. Therefore, we had to find a balance between size and accuracy.
    \item Number of layers added to the core network: The original core network, shown in Figure~\ref{fig:RAM-model}, does not have any hidden fully connected layers between the inputs ($g_t$ and $h_{t-1}$) and the output $h_t$. For traditional inference, adding more layers to the network increases the complexity and computation time. However, for memory-based inference using look-up tables, the depth of the network does not affect the results, since we only care about the inputs and outputs and consider the network as a black-box. Therefore, we tried adding layers to the network to increase the overall accuracy.
\end{itemize}

Figure~\ref{fig:size} shows the accuracy of different numbers of added layers (blue) and different hidden state vector lengths. We identified an elbow point at a length of 48, but we opted for a length of 64 for greater stability.

\subsubsection{Quantization}
We applied mixed-precision quantization to the network in order to significantly reduce the size of the look-up table. Originally, each element in the network's arrays was a 32-bit floating point, and the hidden state vector $h$ was fixed to 256 elements.

We strongly quantized both the patch vector $p$ and hidden state vector $h$, optimizing the precision and type for each vector:
\begin{itemize}
    \item Patch vector: we applied 2-bit quantization to $p$ during both training and testing, as this yielded better results than applying it only during testing. The resulting levels of quantization for $p$ are $L=2^{b=2}=4$.
    \item Hidden state vector: we applied quantization only during inference, as we found that the hidden state needs to be precise at the floating point level during training. If instead $h$ is only quantized during inference, the accuracy drop is negligible. We applied extreme quantization, also known as \emph{binarization} \cite{gholami2021survey}, resulting in $L=2^{b=1}=2$ levels.
\end{itemize}

Before quantizing the hidden state vector $h$, we applied a \texttt{Relu1} function to it. We found that clamping the vector between 0 and 1 consistently reduced accuracy drop, likely because $h$ values rarely exceed 1. We applied linear quantization to both vectors, harnessing the formula shown in Eq.~\ref{eq:linear-quantization}:
\newcommand{\xvect}{\mathbf{x}}
\begin{align}\label{eq:linear-quantization}
\frac{(max_\xvect-min_\xvect)}{(2^{b}-1)} \cdot \left[\frac{(x_0-min_\xvect)}{(max_\xvect-min_\xvect)}\cdot (2^{b}-1)\right]
\end{align}

Here, $\xvect \in \mathbb{R}^n$, $max_\xvect$ and $min_\xvect$ are respectively the maximum and minimum values of the vector, $b$ is the number of bits used for quantization, and $x_0$ is the element to be quantized.

Additionally, we quantized the prediction $a$ and location $l$, but no information was lost as we used the minimum number of bits required to represent all possible values. For the MNIST dataset, $a$ ranges from 0 to 9, and $l_i$ ranges from 0 to 27, both within integer range $I$.

Fig.~\ref{fig:quantization} displays the accuracy results for varying quantization levels of $h$ (red) and $p$ (blue). The quantization value ``inf'' represents the performance without quantization.

\subsection{Look-Up Table for Memory-Based Inference}\label{sec:look-up-structure}
\begin{table}[t]
    \begin{center}
        \begin{tabular}{|c||c|c|c|c|c|c|}
            \toprule
            \textbf{Glimpse} & \textbf{$h_{t-1}$} & \textbf{$l_t$} & \textbf{$p_t$} & \textbf{$h_t$} & \textbf{$l_{t+1}$} & \textbf{$a_t$} \\ [0.5ex] 
            \midrule
            \textbf{1} & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
            $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$  \\
            \textbf{N} & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$  \\ [1ex]
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Table structure}
    \label{tab:table-structure}
\end{table}

As previously mentioned on various occasions, the look-up table is supposed to consist of inputs and outputs for each glimpse. In practice, we replaced the input image with the patch vector $p$ and applied quantization to it. In the following sections, we will describe the steps taken to construct the table from the original network and calculate the size of a table based on our baseline.

\subsubsection{Table structure}\label{sec:table-structure}
The table consists of rows of vectors, where each row represents a glimpse, and each vector is the concatenation of inputs and outputs of that glimpse. Specifically, each row of the table is the concatenation, in order, of $h_{t-1}$, $l_t$, $p_t$, $h_t$, $l_{t+1}$, and $a_t$. A sample of the table is presented in Tab.~\ref{tab:table-structure}, where each row has its prediction.

It is important to note that we made a small modification to the network to save the predictions of glimpses that are not the last, in order to have a prediction for each glimpse and save it in the table.

\subsubsection{Building the table}\label{sec:building-table}
To assess the validity of our inference approach, we need to explain the steps taken to build the look-up table. In short, the table contains the inputs and outputs obtained from running the \emph{inference} on the \emph{training} data of the dataset. The following steps were taken to build the table:
\begin{enumerate}
    \item We trained the network with the baseline configuration \ref{tab:hyperparameter-baseline} and saved the weights in a checkpoint file for future inference.
    \item We ran the inference \emph{again} on the \emph{training data}, saving the inputs and the outputs for each glimpse. We needed to have a trained table to use as reference, but we could not save inputs and outputs \emph{while} the network was being trained, as there would be inconsistency in the precision of the predictions: the more the network is trained, the better is the accuracy. Instead, running inference on the training data does not update the network weights, and most importantly the network ``tests'' something that has actually already seen, hence being pretty accurate. The resulting saved data in the table represents therefore an example to be used for inferring new outputs from new inputs never seen before.
    \item Finally, we performed actual memory-based inference on the trained table by using testing data from the dataset and extracting outputs without conducting any additional computations.
\end{enumerate}

\subsubsection{Table size}
To calculate the table size for the MNIST dataset, we first define the row size $S_r$ using Equation \ref{eq:row-size} where $S_h$, $S_l$, $S_p$, and $S_a$ represent the sizes of the hidden state vector, location vector, patch vector, and prediction value respectively:
\begin{equation}\label{eq:row-size}
    S_r = 2 \cdot S_h + 2 \cdot S_l + S_p + S_a
\end{equation}

The hidden vector has $N_h=64$ elements [Tab.~\ref{tab:hyperparameter-baseline}], while the number of elements $N_p$ in the patch vector is obtained using Eq.~\ref{eq:patch-vector-size-channels}. The location vector represents 2 coordinates ($N_l=2$), and the prediction value is a scalar ($N_a=1$). We use quantization levels with of $b_h=1$, $b_p=2$, $b_l=5$, and $b_a=4$ bits for each element. Using Eq.~\ref{eq:bits-times-n}, we calculate the size of each vector $S_i$:
\begin{equation}\label{eq:bits-times-n}
    S_i = b_i \cdot N_i, \quad i \in \{h,l,p,a\}
\end{equation}

Finally, the total number of rows in the table is:
\begin{align}
    N_r &= N_g\cdot N_s \label{eq:rows-num} \\
    N_r &= 60k \cdot 5 = 300k \label{eq:rows-num-number}
\end{align}
Where $N_g$ is the number of glimpses and $N_s$ is the number of training samples ($60k$ for MNIST).

Combining the baseline configuration at Tab.~\ref{tab:hyperparameter-baseline} and these equations, we obtain the total size of trained table:
\begin{align}
    S_t &= N_r \cdot (2 \cdot b_h \cdot N_h + 2 \cdot b_l \cdot N_l + b_p \cdot N_p + b_a \cdot N_a) \label{eq:table-size} \\
    S_t &= 300k \cdot 248 = 70.95Mb = 8.87MB \label{eq:table-size-number}
\end{align}

\subsection{Memory-Based Inference}
The idea of memory-based inference is centered around the term ``memory'', which evokes the notion of a network's memory. This is because, instead of performing matrix multiplications and linear transformations to derive the output from the input, the network simply recalls which output corresponds to which input, and retrieves it from a memorized table.

To delve deeper, the following steps are involved in memory-based inference:
\begin{enumerate}
    \item Look-up: the new input image is compared among all the inputs in the table using a specific distance metric, and the closest input in the table is selected.
    \item Output extraction: the outputs $h_t$ and $l_{t+1}$ from the same row as the selected input are extracted.
    \item Recurrence: since the network is recurrent, the outputs from step 2) are fed back into the table, and steps 1) and 2) are repeated for the number of glimpses specified during training. After 5 glimpses in our case, only the prediction $a_t$ is extracted from the output.
\end{enumerate}

Note that the table does not contain any information about the original time-step saved in each row. During inference, a prediction from the first, second, or last glimpse could be selected without knowledge of which time-step it came from. This is necessary to achieve convergence, as two rows could be related without ever leading to a row with a prediction. This is why in Sec.~\ref{sec:table-structure} we mentioned that mid-step predictions were also saved during table construction.

\subsubsection{Percentage of training data}\label{sec:percentage-data}
The original trained table stores the entire training data of the dataset, resulting in a size of slightly less than $9MB$ [Sec.~\ref{sec:building-table}, Eq.~\ref{eq:table-size-number}]. However, it may be beneficial to reduce the table size by shrinking it directly after building it. To achieve this, we randomly extracted different percentages of rows from the original trained table using a uniform distribution, and tested memory-based inference (MBI) on the resulting tables. We reported the results at Sec.~\ref{sec:results-percentage}.

\subsection{Distance Metric for MBI}
To efficiently compare input vectors and find the closest match in the table, we utilized a distance metric that could be easily implemented in hardware. After comparing several distance metrics, we found that the Manhattan distance metric provided a good balance of accuracy and simplicity.

\newcommand{\qvect}{\mathbf{q}}
\newcommand{\tvect}{\mathbf{t}}
\newcommand{\qmatr}{\mathbf{Q}}
Let $\qvect$ and $\tvect$ be the vector already saved in the table and the input vector, respectively, both of length $n$. The power of 2 distance metric computes the sum of squared differences between corresponding elements of $\qvect$ and $\tvect$, while the Manhattan distance metric calculates the sum of absolute differences. The formulas for these two metrics are given by Eqs.~\ref{eq:euclidean} and \ref{eq:manhattan}:
\begin{align}
    E_d(\qvect,\tvect) &= \sum_{i=1}^n (q_i - t_i)^2 \label{eq:euclidean} \\
    M_d(\qvect,\tvect) &= \sum_{i=1}^{n}|q_{i} - t_{i}| \label{eq:manhattan}
\end{align}

\subsubsection{Bayesian Optimization}
As described in Sec.~\ref{sec:look-up-structure}, the input to the table consists of the first three entries of Tab.~\ref{tab:table-structure}: $h_{t-1}$, $l_t$, and $p_t$, which are concatenated into a single vector. The distance metric shown in Eq.~\ref{eq:manhattan} is applied to the entire input vector. Specifically, if we use $\qvect$ to represent the table vector and $\tvect$ to represent the target vector (i.e., the new input), we can extract the row with the closest input using Eq.~\ref{eq:closest-input}:
\begin{equation}\label{eq:closest-input}
    D_{clos}(\qmatr,\tvect) = \operatorname*{argmin}_i \{M_{d}(\qvect_i,\tvect)\}
\end{equation}

Here, $\qmatr$ represents the set of rows in the table, and $\qvect_i$ represents a single vector in the set. However, this distance metric does not consider the relative importance of each input in the table. Specifically, we're assigning equal weight to the hidden state, location, and patch vectors, even though they may not be equally important for classification. To address this issue, we can define a new distance metric $D$ that takes these differences into account:
\begin{equation}\label{eq:weighted-manhattan}
    D = \frac{a \cdot M_d(\mathbf{p},\tvect) + b \cdot M_d(\mathbf{h},\tvect) + c \cdot M_d(\mathbf{l},\tvect)}{a+b+c}
\end{equation}

Here, $a$, $b$, and $c$ are real numbers between 1 and 100. However, we cannot determine the importance of each input vector in advance, nor can we manually try all possible combinations. Therefore, we use Bayesian Optimization to find optimal weights that result in better overall inference accuracy. Specifically, we maximize the Memory-Based Inference function $MBI$ by finding the optimal $a$, $b$, and $c$ values using Eq.~\ref{eq:bo}.
\begin{equation}\label{eq:bo}
    \max_{a,b,c} \{MBI(a, b, c)\}
\end{equation}

The resulting improvement is reported at Sec.~\ref{sec:results-bo}.

\subsubsection{Simulated noise}
After fixing the weights through BO, we added a Gaussian noise with a variable standard deviation to the distance metric to simulate natural hardware noise:
\begin{equation}\label{eq:gaussian-noise}
    G_N \sim \mathcal{N}(0, \sigma^2)
\end{equation}

By applying Eq.~\ref{eq:gaussian-noise} to the Manhattan distance metric [Eq.~\ref{eq:manhattan}], we obtain:
\begin{equation}\label{eq:noised-manhattan}
    M^*_d(\qvect, \tvect) = M_d(\qvect,\tvect) \cdot G_N
\end{equation}

Combining Eq.~\ref{eq:weighted-manhattan} with Eq.~\ref{eq:noised-manhattan}, we derive the final distance metric for memory-based inference:
\begin{equation}\label{eq:noised-distance}
    D = \frac{a \cdot M^*_d(\mathbf{p},\tvect) + b \cdot M^*_d(\mathbf{h},\tvect) + c \cdot M^*_d(\mathbf{l},\tvect)}{a+b+c}
\end{equation}

As expected, by increasing the standard deviation, we found a decrease in accuracy. The results are illustrated at Sec.~\ref{sec:results-noise}.

\subsection{Other Datasets}

In addition to using the MNIST dataset for our experiments, we also tested the effectiveness of our model on two other datasets: FashionMNIST and CIFAR-10. The results of these evaluations are outlined in Section~\ref{sec:results-datasets}. It is crucial to note that we did not exhaustively explore the full range of possibilities within these datasets. Rather, we applied the same baseline used for MNIST to these other datasets, recognizing that it may be necessary to adjust hyperparameters differently for each specific dataset.

==> sections/results.tex <==
\section{Simulation Results}\label{sec:results}

The following section presents the results of Memory-Based Inference applied to the trained table previously described. We describe the significance of the improvements made for each step of the methodology.

\subsection{Training Data Percentage}\label{sec:results-percentage}
\begin{table}[t]
    \begin{center}
        \begin{tabular}{|c||c|c|}
            \toprule
            \textbf{Training data} & \textbf{Acc. without BO} & \textbf{Acc. with BO} \\ [0.5ex] 
            \midrule
            \textbf{15\%} & $81.47\%$ & $84.57\%$\\
            \textbf{30\%} & $83.85\%$ & $87.74\%$ \\
            \textbf{50\%} & $85.22\%$ & $88.79\%$ \\
            \textbf{70\%} & $85.69\%$ & $89.40\%$ \\
            \textbf{90\%} & $86.05\%$ & $89.41\%$ \\
            \textbf{100\%} & $85.05\%$ & $89.19\%$ \\ 
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Accuracy for each subset of training data}
    \label{tab:percentage-accuracy}
\end{table}

We employed MBI on different percentages of the training data obtained from the original table, as detailed in Section~\ref{sec:percentage-data}.

Our findings revealed that the accuracy plateaued at 50\% of the data, indicating that significant improvement was not observed beyond this point. This suggests that there may be a general limit to the amount of training data that can be utilized for making predictions.

To provide a comprehensive view of the results, we reported the accuracy for each portion of the training data in Tab.~\ref{tab:percentage-accuracy}, both with and without Bayesian Optimization. The elbow point can be easily spotted in Fig.~\ref{fig:bo}, where both curves demonstrate a similar pattern, with the accuracy steadily increasing up to 50\% of the training data and then leveling off.

\subsection{Bayesian Optimization}\label{sec:results-bo}
\begin{table}[t]
    \begin{center}
        \begin{tabular}{|c||c|c|c|c|}
            \toprule
            \textbf{Training data} & \textbf{Accuracy} & \textbf{a} & \textbf{b} & \textbf{c} \\ [0.5ex] 
            \midrule
            \textbf{15\%} & $84.57\%$ & $30.930$ & $15.529$ & $10.142$ \\
            \textbf{30\%} & $87.74\%$ & $100.00$ & $22.514$ & $86.900$  \\
            \textbf{50\%} & $88.79\%$ & $55.365$ & $11.652$ & $36.038$  \\
            \textbf{70\%} & $89.40\%$ & $63.545$ & $19.626$ & $48.075$  \\
            \textbf{90\%} & $89.41\%$ & $96.102$ & $35.669$ & $32.637$  \\
            \textbf{100\%} & $89.19\%$ & $85.985$ & $43.005$ & $92.388$  \\ 
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Optimal weights with BO}
    \label{tab:bo-weights}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.80\linewidth]{resources/graphs/bo.png}
    \caption{Accuracy with and without BO}
    \label{fig:bo}
\end{figure}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.38\linewidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{resources/graphs/bo.png}
%         \caption{Accuracy with and without BO}
%         \label{fig:bo}
%     \end{subfigure}%
%     \begin{subfigure}{0.38\linewidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{resources/graphs/noises.png}
%         \caption{Accuracy drop with Gaussian noise}
%         \label{fig:noise}
%     \end{subfigure}
%     \caption{}
%     \label{fig:graphs-bo-noise}
% \end{figure*}

By applying Bayesian Optimization to the weighted Manhattan distance metric [Eq.\ref{eq:weighted-manhattan}], we were able to observe a constant improvement in accuracy for each percentage of training data, with a 3\% to 4\% increase in overall accuracy [Fig.\ref{fig:bo}]. To provide further insight into our results, we present in Tab.~\ref{tab:bo-weights} the values of $a$, $b$, and $c$ that were derived by BO for each percentage of training data.

\subsection{Noise Simulation}\label{sec:results-noise}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.80\linewidth]{resources/graphs/noises.png}
    \caption{Accuracy drop with Gaussian noise}
    \label{fig:noise}
\end{figure}

When we also applied Gaussian noise [Eq.~\ref{eq:noised-distance}], we observed an elbow point at a standard deviation of approximately $\sigma=1.0$. Beyond this point, the drop in accuracy follows a linear trend with respect to $\sigma$. Additionally, we noticed that the overall accuracy using 50\% or 100\% of the data is nearly identical after the elbow point [Fig.~\ref{fig:noise}]. The only discernible difference between the two can be deduced to be network's instability.

\subsection{Other Datasets}\label{sec:results-datasets}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.80\linewidth]{resources/graphs/histogram.png}
    \caption{Accuracy drop with other datasets}
    \label{fig:histogram}
\end{figure}

We reported here the accuracy drop when transitioning from standard inference to MBI across various datasets. A summary of our findings can be seen in Figure~\ref{fig:histogram}.

Notably, the quantized case demonstrates consistent accuracy drops across the different datasets. This suggests that our model is highly robust and capable of generalizing well to diverse data distributions, indicating its potential as an effective approach for various machine learning tasks.
